On Unifying Randomized Methods For Inverse Problems

This work unifies the analysis of various randomized methods for solving linear and nonlinear inverse problems by framing the problem in a stochastic optimization setting. By doing so, we show that many randomized methods are variants of a sample average approximation. More importantly, we are able to prove a single theoretical result that guarantees the asymptotic convergence for a variety of randomized methods. Additionally, viewing randomized methods as a sample average approximation enables us to prove, for the first time, a single non-asymptotic error result that holds for randomized methods under consideration. Another important consequence of our unified framework is that it allows us to discover new randomization methods. We present various numerical results for linear, nonlinear, algebraic, and PDE-constrained inverse problems that verify the theoretical convergence results and provide a discussion on the apparently different convergence rates and the behavior for various randomized methods.

==> linear_nonasymptotic_theory.tex <==
\section{Linear non-asymptotic theory}
\label{appendix:linear_nonasymptotic}

% The linear case - keep just in case
The proof of a non-asymptotic error bound for $\tilde{\ub}^{\text{\normalfont{MAP}}}_N$ \eqnref{independent_SA_nonasymptotic} 
in the linear case follows 
standard perturbation analysis for linear systems of equations \cite{QuarteroniSaccoSaleri2006}.
Particularly, 
for a linear system of the form $\Mb\ub = \rbb$ with solution $\ub^*$,
the perturbed system $\LRp{\Mb + \Delta \Mb}\ub = \LRp{\rbb + \Delta \rbb}$
with solution $\tilde \ub$ has relative error satisfying 
\begin{equation}
    \eqnlab{linear_perturb}
    \frac{\norm{\ub^* - \tilde{\ub}}}{\norm{\ub^*}} \leq 
    \frac{\kappa (\Mb)}{1 - \kappa (\Mb)\frac{\norm{\Delta \Mb}}{\norm{\Mb}}}
    \LRs{\frac{\norm{\Delta \Mb}}{\norm{\Mb}} + 
    \frac{\norm{\Delta \rbb}}{\norm{\rbb}}}
\end{equation}
under the condition that $\kappa (\Mb)\frac{\norm{\Delta \Mb}}{\norm{\Mb}} < 1$. We prove two intermediate results to arrive at the 
final non-asymptotic error bound.
\newcommand{\Ab}{\bs{A}}
\newcommand{\Bb}{\bs{B}}
\newcommand{\xb}{\bs{x}}
\begin{proposition}
    \propolab{matrix_norm_inequality}
    Let $\Mb = \Ab + \Bb$ where $\Ab, \Bb, \Mb \in \R^{n \times n}$ are symmetric positive semi-definite (SPSD) matrices. 
    Then 
    \begin{equation*}
    \norm{\Mb}_\infty \geq n \norm{\Ab}_\infty \text{ and } \norm{\Mb}_\infty \geq n \norm{\Bb}_\infty. 
    \end{equation*}
\end{proposition}
\begin{proof}
    Without loss of generality, we first show that 
    \begin{equation}
        \eqnlab{matrix_2_norm_ineq}
        \norm{\Mb}_2 \geq \norm{\Ab}_2
    \end{equation}
    Recall that the induced 2-norm of a matrix is defined as
    \begin{equation*}
        \norm{\Mb}_2 := \max_{\norm{\xb} = 1} \norm{\Mb \xb}_2= \max_{\norm{\xb} = 1} x^T \Mb x,
    \end{equation*}
    where $\xb \in \R^n$. Suppose without loss of generality that $\norm{\Ab}_2 > \norm{\Mb}_2$. 
    Then,
    \begin{equation*}
        \xb^T \Ab \xb > \xb^T \Mb \xb = \xb^T \Ab \xb + \xb^T \Bb \xb. 
    \end{equation*}
    This implies that 
    \begin{equation*}
         \xb^T \Bb \xb < 0, 
    \end{equation*}
    a contradiction since $\Bb$ is SPSD. 
    Now, also recall the following relationship between matrix norms found in \cite{trefethen1997numerical}:
    \begin{equation}
        \eqnlab{infinity_two_inequality}
        \frac{1}{\sqrt{n}}\norm{\Ab}_\infty \leq \norm{\Ab}_2  \leq \sqrt{n} \norm{\Ab}_\infty.
    \end{equation}
    Applying \eqnref{infinity_two_inequality} to \eqnref{matrix_2_norm_ineq} twice completes the proof.
\end{proof}
\begin{proposition}
  \propolab{LHS_perturb}
    Let $\Mb := \A^T \L^{-1}\A + \sC^{-1}$ and $\LRp{\Mb + \Delta \Mb} := \A^T \Sn \A + \Ln$ 
    where $\Sn$ and $\Ln$ are defined in \eqnref{SA_definitions} and $\epsb$ and $\lamb$ are subgaussian random variables.
    Then the following holds:
    \begin{equation*}
        \frac{\norm{\Delta \Mb}_\infty}{\norm{\Mb}_\infty} \leq 2n \tol \quad
        \text{ w.p. at least }  
        1 - 4 \zeta \LRp{\N, \tol}. 
    \end{equation*}
\end{proposition}
\begin{proof}
  It is clear that, 
  \begin{equation*}
    \Delta \Mb = \A^T\LRp{\Sn - \L^{-1}} \A + \LRp{\Ln - \sC^{-1}}.
  \end{equation*}
  Then, 
  \begin{subequations}
    \begin{align*}
      \norm{\Delta \Mb}_\infty &= \norm{\A^T\LRp{\Sn - \L^{-1}} \A + \LRp{\Ln - \sC^{-1}} }_\infty \\
                        &\leq \norm{\A^T\LRp{\Sn - \L^{-1}} \A}_\infty + \norm{\LRp{\Ln - \sC^{-1}}}_\infty.
    \end{align*}
  \end{subequations}
  From Proposition \proporef{outer_product},
  \begin{subequations}
    \eqnlab{mb_bounds}
    \begin{align}
      \eqnlab{model_perturb}
      &\norm{\A^T\LRp{\Sn - \L^{-1}} \A}_\infty \leq \tol \norm{\A^T\L^{-1}\A}_\infty\quad \text{ w.p. at least } 1 - 2 \zeta \LRp{\N, \tol},\\
      \eqnlab{prior_perturb}
      &\norm{\LRp{\Ln - \sC^{-1}}}_\infty \leq \tol \norm{\sC^{-1}}_\infty \hspace{2.2cm} \text{ w.p. at least } 1 - 2 \zeta \LRp{\N, \tol}.
    \end{align}
  \end{subequations}
  Since both $\A^T\L^{-1}\A$ and $\sC^{-1}$ are SPSD and recalling that $\Mb \in \R^{n \times n}$, 
  Proposition \proporef{matrix_norm_inequality} implies,
  \begin{align*}
    \norm{\Mb}_\infty &\geq \frac{1}{n} \norm{\A^T\L^{-1}\A}_\infty \text{ and } \norm{\Mb}_\infty \geq \frac{1}{n} \norm{\sC^{-1}}_\infty.
  \end{align*}
  It follows that 
  \begin{equation*}
    \norm{\Mb}_{\infty} \geq \frac{1}{2n} \norm{\A^T\L^{-1}\A}_\infty + \frac{1}{2n} \norm{\sC^{-1}}_\infty.
  \end{equation*}
  Finally, 
  \begin{align*}
    \frac{\norm{\Delta \Mb}_\infty}{\norm{\Mb}_\infty} &\leq 
        \tol \frac{\norm{\A^T\L^{-1}\A}_\infty + \norm{\sC^{-1}}_\infty}{\norm{\Mb}_\infty} 
        \leq 2n \tol \frac{\norm{\A^T\L^{-1}\A}_\infty + \norm{\sC^{-1}}_\infty}{\norm{\A^T\L^{-1}\A}_\infty + \norm{\sC^{-1}}_\infty} 
        = 2n \tol \\
        & \text{ w.p. at least } 1 - 4 \zeta \LRp{\N, \tol}.
  \end{align*}
\end{proof}
Note that in the preceding proof, \eqnref{model_perturb} and \eqnref{prior_perturb} have different
constants buried in each $\zeta\LRp{\N,\tol}$ term. However, this does not affect the
convergence rate with respect to $\N$ and can easily be rectified by taking $c = \min\LRc{c_1, c_2}$ where
$c_1$ is the constant associated with \eqnref{model_perturb} and $c_2$ is the
constant associated with \eqnref{prior_perturb}. Such details will not be explicitly addressed in the remaining
proofs as we can always pick an appropriate constant such that the $\zeta$ terms can be additively combined while
maintaining the appropriate inequalities. 
\begin{proposition}
  \propolab{RHS_perturb}
    Let $\rbb := \A^T \L^{-1} \db + \sC^{-1} \ub_0$ and 
    $\LRp{\rbb + \Delta \rbb} := \A^T \Sn \LRp{\db + \sigbarN} + \Ln \LRp{\ub_0 + \delbarN}$.
    Then the following holds:
    \begin{subequations}
    \begin{align*}
        \frac{\norm{\Delta \rbb}_\infty}{\norm{\rbb}_\infty} 
          & \leq \tol \frac{\norm{\A^T \L^{-1}}_\infty\LRp{\LRp{1 + \tol}\norm{\L^{\half}}_\infty + \norm{\db}_\infty} +
            \norm{\sC^{-1}}_\infty \LRp{\LRp{1 + \tol}\norm{\sC^{\half}}_\infty  + \norm{\ub_0}_\infty}}{\norm{\A^T \L^{-1} \db + \sC^{-1} \ub_0}_\infty}\\
        &\text{ w.p. at least }  
          1 - 10 \zeta \LRp{\N, \tol}
    \end{align*}
  \end{subequations}
\end{proposition}
\begin{proof}
  \begin{subequations}
    \begin{align*}
      \norm{\Delta \rbb}_\infty &= \norm{\A^T \Sn \LRp{\db + \sigbarN} + \Ln \LRp{\ub_0 + \delbarN}
                            - \LRp{A^T \L^{-1}\db + \sC^{-1}\ub_0}}_\infty \\
                         & \leq \norm{\A^T \LRp{\Sn - \L^{-1}}\db}_\infty + \norm{\LRp{\Ln - \sC^{-1}}\ub_0}_\infty
                            + \norm{A^T\Sn\sigbarN}_\infty + \norm{\Ln\delbarN}_\infty
    \end{align*}
  \end{subequations}
  Applying Proposition \proporef{outer_product} to the first two terms,
  \begin{subequations}
    \begin{align*}
      &\norm{\A^T \LRp{\Sn - \L^{-1}}\db}_\infty + \norm{\LRp{\Ln - \sC^{-1}}\ub_0}_\infty \leq
        \tol \LRp{\norm{\A^T\L^{-1}}_\infty\norm{\db}_\infty + \norm{\sC^{-1}}_\infty \norm{\ub_0}_\infty} \\
      & \quad \text{w.p at least } 1 - 4 \zeta\LRp{\N, \tol}. 
    \end{align*}
  \end{subequations}
  The remaining terms can be bounded using both Propositions \proporef{zero_mean} and \proporef{outer_product}.
  \begin{subequations}
    \begin{align*}
      \norm{\A^T\Sn \sigbarN}_\infty &= \norm{A^T \LRp{\L^{-1} + \LRp{\Sn - \L^{-1}}}\sigbarN}_\infty  \\
                              &\leq \norm{A^T \L^{-1}\sigbarN}_\infty +  \norm{\A^T \LRp{{\Sn - \L^{-1}}}\sigbarN}_\infty  \\
                              &\leq \norm{\sigbarN}_\infty \LRp{\norm{A^T \L^{-1}}_\infty +  \norm{\A^T \LRp{\Sn - \L^{-1}}}_\infty} \\
                              &\leq \tol \norm{\L^{\half}}_\infty \LRp{\norm{A^T \L^{-1}}_\infty +  \norm{\A^T \LRp{\Sn - \L^{-1}}}_\infty}\\ 
                              &\quad \quad \text{ w.p. at least } 1 - \zeta\LRp{\N, \tol}.
    \end{align*}
  \end{subequations}
  This last inequality arises from an application of Proposition \proporef{zero_mean}. Making use once more of
  Proposition \proporef{outer_product} along with the union bound,
  \begin{subequations}
    \begin{align*}
      \norm{\A^T\Sn \sigbarN}_\infty &\leq \LRp{1 + \tol}\tol \norm{\L^{\half}}_\infty \norm{\A^T \L^{-1}}_\infty \\
                              &\quad \quad \text{ w.p. at least } 1 - 3\zeta\LRp{\N, \tol}.
    \end{align*}
  \end{subequations}
  Similarly, it can be shown that 
  \begin{subequations}
  \begin{align*}
    \norm{\Ln\delbarN}_\infty &\leq \LRp{1 + \tol}\tol \norm{\sC^{\half}}_\infty \norm{\sC^{-1}}_\infty \\
        &\quad \quad \text{ w.p. at least } 1 - 3\zeta\LRp{\N, \tol}.
  \end{align*}
  \end{subequations}
  Dividing by $\norm{\rbb}_\infty$ completes the proof.
\end{proof}

As a direct result of propositions \proporef{LHS_perturb} and \proporef{RHS_perturb}
and standard perturbation analysis for linear systems \eqnref{linear_perturb}, 
we can write down a non-asymptotic bound on the error due to the general randomization strategy proposed.

\begin{corollary}
  \corolab{nonasymptotic_convergence}
  Letting $\Mb = \A^T \L^{-1}\A + \sC^{-1}$, 
  \begin{subequations}
    \eqnlab{nonasymptotic_convergence}
  \begin{align*}
  \frac{\norm{\ub^* - \tilde{\ub}}}{\norm{\ub^*}} &\leq
  \frac{\kappa \LRp{\Mb}}{1 - 2\tol \kappa \LRp{\Mb}}
    \LRs{2 + \frac{\norm{\A^T \L^{-1}}\LRp{1 + \tol + \norm{\db}} +
            \norm{\sC^{-1}} \LRp{1 + \tol + \norm{\ub_0}}}{\norm{\A^T \L^{-1} \db + \sC^{-1} \ub_0}}}\tol \\
    & \text{ w.p. at least } 1 - 12 \zeta_2 \LRp{\N, \tol} - \zeta_1 \LRp{\L, \N, k, \tol} -
      \zeta_1 \LRp{\sC, \N, n, \tol}.
  \end{align*}
\end{subequations}
\end{corollary}
\begin{proof}
  The proof follows from propositions \proporef{LHS_perturb}, \proporef{RHS_perturb}, and the union bound.
\end{proof}

\begin{corollary}
  Consider the case where the data and prior means are not randomized.
  That is, let $\delbarN = \sigbarN \equiv 0$. Then
  \begin{subequations}
    \eqnlab{nonasymptotic_convergence_no_mean_rand}
  \begin{align*}
  \frac{\norm{\ub^* - \tilde{\ub}}}{\norm{\ub^*}} &\leq
  \frac{\kappa \LRp{\Mb}}{1 - 2\tol \kappa \LRp{\Mb}}
    \LRs{2 + \frac{\norm{\A^T \L^{-1}}\norm{\db} +
            \norm{\sC^{-1}} \norm{\ub_0}}{\norm{\A^T \L^{-1} \db + \sC^{-1} \ub_0}} }\tol \\
    & \text{ w.p. at least } 1 - 8 \zeta_2 \LRp{\N, \tol}.
  \end{align*}
\end{subequations}
\end{corollary}

==> notes_macros.tex <==
\newcommandx{\question}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\add}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
\newcommandx{\improve}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
\newcommandx{\remove}[2][1=]{\todo[linecolor=yelllow,backgroundcolor=yellow!10,bordercolor=red,#1]{#2}}

%%%--------------------------------------------------------------------

% color
\newcommand{\mygreen}[1]{{\color[rgb]{0,.65,0} #1}}
\newcommand{\mywhite}[1]{{\color[rgb]{1.0,1.0,1.0} #1}}
\newcommand{\myred}[1]{{\color[rgb]{0.65,0.0,0.0} #1}}
\newcommand{\myblue}[1]{{\color[rgb]{0.0,0.0,1.0} #1}}
\newcommand{\mygray}[1]{{\color[rgb]{.15,.35,.60} #1}}
\newcommand{\mythemec}[1]{{\color[RGB]{51,108,121} #1}}
\newcommand{\mydarkred}[1]{{\color[rgb]{.6,.1,.1} #1}}
\newcommand{\mydarkblue}[1]{{\color[rgb]{.1,.1,.9} #1}}
\newcommand{\mygreenback}[1]{{\color[rgb]{.75,1,.75} #1}}
\newcommand{\myorange}[1]{{\color[rgb]{.76,.39,.13} #1}}
\newcommand{\mygrass}[1]{{\color[rgb]{.19,.64,.13} #1}}
\newcommand{\mysierp}[1]{{\color[RGB]{209,28,209} #1}}

\DeclareSymbolFontAlphabet{\mathbb}{AMSb}
\DeclareSymbolFontAlphabet{\mathbbl}{bbold}

==> tables/1d_deconvolution.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{ |l|l|l|l|l| }
    \hline
    \multirow{2}{*}{Method} & \multicolumn{4}{c|}{Relative error ($\%$)}   \\ \cline{2-5}
      & N = 10& N = 100& N = 1000& N = 10000\\ \cline{2-5}
    \hline
    \text{RMAP}  & 7.49 & 2.33 & 0.74 & 0.23  \\ \cline{1-5}
    \text{RMA}  & 48.85 & 6.70 & 1.39 & 0.59  \\ \cline{1-5}
    \text{RMA+RMAP}  & 50.84 & 5.84 & 2.10 & 0.69  \\ \cline{1-5}
    \text{RS\_U1}  & 38214006.97 & 28298959.46 & 549.22 & 31.51  \\ \cline{1-5}
    \text{RS}  & 948.19 & 305.97 & 107.57 & 30.51  \\ \cline{1-5}
    \text{ENKF}  & 880.15 & 329.65 & 100.17 & 32.18  \\ \cline{1-5}
  \end{tabular}
  \caption{Computed relative error for the 1D Deconvolution problem using different randomized approaches}
  \label{Table:1D_Deconv}
\end{table}

